What Are the Odds? Improving the foundations of Statistical Model Checking

Markov decision processes (MDPs) are a fundamental model for decision making under uncertainty. They exhibit non-deterministic choice as well as probabilistic uncertainty. Traditionally, verification algorithms assume exact knowledge of the probabilities that govern the behaviour of an MDP. As this assumption is often unrealistic in practice, statistical model checking (SMC) was developed in the past two decades. It allows to analyse MDPs with unknown transition probabilities and provide probably approximately correct (PAC) guarantees on the result. Model-based SMC algorithms sample the MDP and build a model of it by estimating all transition probabilities, essentially for every transition answering the question: ``What are the odds?'' However, so far the statistical methods employed by the state of the art SMC algorithms are quite naive. Our contribution are several fundamental improvements to those methods: On the one hand, we survey statistics literature for better concentration inequalities; on the other hand, we propose specialised approaches that exploit our knowledge of the MDP. Our improvements are generally applicable to many kinds of problem statements because they are largely independent of the setting. Moreover, our experimental evaluation shows that they lead to significant gains, reducing the number of samples that the SMC algorithm has to collect by up to two orders of magnitude.

==> sections/20_ideas.tex <==
\section{Ideas}


	\subsection{Breaking the union bound}

	Our general approach is: Probability of estimating any probability wrong = Sum of estimating any particular probability wrongly.

	Observe that when we only care about the, e.g., maximal value w.r.t.\ to any objective, we actually do not need every transition to be precise with $1 - \delta$ probability.
	Instead, we only need that for each strategy, the probability to reach a wrongly estimated transition is at most $\delta$.

	Observe: Let $S_1$ and $S_2$ two SCCs that are incomparable in the strict topological ordering (this just means there is no path from $S_1$ to $S_2$ and none vice-versa).
	Then, any path that reaches a state in $S_1$ will never reach a state in $S_2$ and vice versa.
	\todo{... and now I don't know what to write. The idea is that we can use the same delta for $S_1$ and $S_2$, since their errors cannot add up - if you enter $S_1$ you cannot make a mistake in $S_2$ and vice versa}

	Attempt (for MC here, MDP should be similar):

	Let $\MC=(\States,P)$ be a Markov Chain with $S_1,S_2$ incomparable SCCs as above. Let $\delta_{s,s'}$ denote the error tolerance for $P(s,s')$ and $I=(\States,\hat{P})$ the interval Markov Chain constructed from some data set over $\MC$.
	We define a partition $T_0\cup T_1\cup T_2$ on the set of transitions in the Markov Chain: $T_i = \left\{(s,s') \mid P(s,s')>0 \text{ and }\{s,s'\}\cap S_i\neq\emptyset\right\}$ for $i\in\{1,2\}$ and $T_0$ containing all remaining transitions, i.e., $T_0 = \left\{(s,s') \mid P(s,s')>0\right\} \setminus \{T_1\cup T_2\}$.
	For ease of notation we further define $\delta_{T_i}=\sum_{(s,s')\in T_i} \delta_{s,s'}$ for $i\in\{0,1,2\}$.

	We first note that the following statements hold with probability at least $1-\delta_{T_0}$, and $1-\delta_{T_1}$, and $1-\delta_{T_2}$, respectively:
	\begin{align}
		&\forall (s,s')\in T_0\colon P(s,s')\in \hat{P}(s,s') \label{eq:transitions0} \\
		&\forall (s,s')\in T_1\colon P(s,s')\in \hat{P}(s,s') \label{eq:transitions1} \\
		&\forall (s,s')\in T_2\colon P(s,s')\in \hat{P}(s,s') \label{eq:transitions2}
	\end{align}
	This is by construction of $I$ and the correctness probability is obtained by applying the the union bound.

	Now consider a path $\infinitepath=s_0s_1\dots\in\Infinitepaths<\MC>$ of $\MC$. Note that by definition of $S_1$ and $S_2$, it cannot be that $\infinitepath$ visits $S_1$ and $S_2$. We want to compute the of encountering a transition $(s,s')$ in $\infinitepath$ for which $P(s,s')\not\in \hat{P}(s,s')$:
	\begin{align*}
		&\; Pr(\exists ss'\in\infinitepath \colon P(s,s')\not\in \hat{P}(s,s') )\\
		= &\; Pr(\exists ss'\in\infinitepath \colon P(s,s')\not\in \hat{P}(s,s') \mid \infinitepath\models\neg\lozenge(S_1\cup S_2)) \ProbabilityMC<\MC, s_0>(\neg \lozenge(S_1\cup S_2))  \\
		&+ Pr(\exists ss'\in\infinitepath \colon P(s,s')\not\in \hat{P}(s,s') \mid \infinitepath\models\lozenge S_1) \ProbabilityMC<\MC, s_0>(\lozenge S_1)\\
		&+ Pr(\exists ss'\in\infinitepath \colon P(s,s')\not\in \hat{P}(s,s') \mid \infinitepath\models\lozenge S_2)\ProbabilityMC<\MC, s_0>(\lozenge S_2)\\
		\leq &\; \delta_{T_0}\ProbabilityMC<\MC, s_0>(\neg \lozenge(S_1\cup S_2)) \\
		&+ (\delta_{T_0}+\delta_{T_1})\ProbabilityMC<\MC, s_0>(\lozenge S_1) \\
		&+ (\delta_{T_0}+\delta_{T_2})\ProbabilityMC<\MC, s_0>(\lozenge S_2) \\
		\leq &\; \delta_{T_0}+\max\{\delta_{T_1},\delta_{T_2}\}
	\end{align*}
	\textcolor{red}{PW: This is not quite there. However, I keep running into walls here as well... Most of the time the issue is something like this: SOTA Model-SMC proves that with probability $1-\delta$ that all $\rho$ are estimated correctly SIMULTANEOUSLY. When not splitting $\delta$ over SCCs, we can only prove that for every $\rho$ that it is estimated correctly with probability $1-\delta$. But we cannot prove that these events coincide - e.g. it might be that $\rho_1$ and $\rho_2$ are estimated correctly w/ prob $1-\delta_1$ and $1-\delta_2$, but the prob that both are estimated correctly may be $1-2\delta$. the best we can do is to show that they are independent, reducing it to $(1-\delta_1)(1-\delta_2)$ which is the same as splitting over states (but using independence instead of union bound). everything below is a pile of more failed attempts and not necessarily structured.}

	Importantly, by construction of $T_1$ and $T_2$ together with the properties of SCCs, $\finitepath$ may not contain transitions from $T_1$ \emph{and} $T_2$. Thus, the statement
	\begin{equation}
		 \forall ss'\in \finitepath\colon P(s,s')\in \hat{P}(s,s') \label{eq:path_correct}
	\end{equation}
	follows from combining either \Cref{eq:transitions0} and \Cref{eq:transitions1}, or \Cref{eq:transitions0} and \Cref{eq:transitions2}. Only a subset of these may suffice for some $\finitepath$, but one pair definitely proves the statement for any $\finitepath$.
	Therefore, by applying the union bound we obtain that for all $\finitepath=s_0s_1\dots s_n\in\Finitepaths<\MC>$ \Cref{eq:path_correct} holds with probability at least $1-\sum_{(s,s')\in T_0} \delta_{s,s'}-\max \left\{\sum_{(s,s')\in T_1} \delta_{s,s'},\sum_{(s,s')\in T_2} \delta_{s,s'}\right\}$


	Because of the SCC property we can partition $\Finitepaths<\MC,g>$ into three sets:
	\begin{itemize}
		\item $\Finitepaths<\MC,g,1>$ containing all paths visiting $S_1$
		\item $\Finitepaths<\MC,g,2>$ containing all paths visiting $S_2$
		\item $\Finitepaths<\MC,g,0>$ containing all paths visiting neither $S_1$ nor $S_2$
	\end{itemize}
	Therefore we can write:
	\begin{align*}
	\ProbabilityMC<\MC, s_0>(\lozenge g) =& \sum_{\finitepath\in\Finitepaths<\MC,g>} \ProbabilityMC<\MC, s_0>(\finitepath) \\
		=& \sum_{\finitepath\in\Finitepaths<\MC,g,0>} \ProbabilityMC<\MC, s_0>(\finitepath)
		+ \sum_{\finitepath\in\Finitepaths<\MC,g,1>} \ProbabilityMC<\MC, s_0>(\finitepath)
		+ \sum_{\finitepath\in\Finitepaths<\MC,g,2>} \ProbabilityMC<\MC, s_0>(\finitepath)
	\end{align*}

	In the Interval MC $I$ we similarly estimate the lower bound of the goal probability: \todo{actually define probability measure for interval markov systems in prelims}
	\begin{align*}
		\ProbabilityMC<I, s_0>^-(\lozenge g) =& \min_{\MC^-\in [I]}\sum_{\finitepath\in\Finitepaths<\MC^-,g>} \ProbabilityMC<\MC^-, s_0>(\finitepath) \\
		=& \min_{\MC^-\in [I]}\Bigg(\sum_{\finitepath\in\Finitepaths<\MC,g,0>}\ProbabilityMC<\MC^-, s_0>(\finitepath)
		+ \sum_{\finitepath\in\Finitepaths<\MC,g,1>} \ProbabilityMC<\MC^-, s_0>(\finitepath)
		+ \sum_{\finitepath\in\Finitepaths<\MC,g,2>} \ProbabilityMC<\MC^-, s_0>(\finitepath)\Bigg)
	\end{align*}
	and analogously for $\ProbabilityMC<I, s_0>^+$.
	Notice that from $ \Finitepaths<\MC^-, s_0>= \Finitepaths<\MC, s_0>$ because grey-box.

	Let $\finitepath_1\in\Finitepaths<\MC,g,1>$ be an arbitrary finite path to $g$ through $S_1$. By definition of SCCs is must be of the form $\finitepath=s_0s_1\dots s_{i_1} \dots s_{i_1} \dots s_n$ with $0<k\leq m<n$ and $s_n=g$, where $s_i \in S_1$ if $i_1\leq i\leq i_2$ and otherwise $s_i \in S\setminus \{S_1\cup S_2\}$. Therefore we can write
	\begin{equation}
		\ProbabilityMC<\MC, s_0>(\finitepath_1) = \ProbabilityMC<\MC, s_0>(s_0\dots  s_{i_1}) \cdot \ProbabilityMC<\MC, s_0>(s_{i_1}\dots s_{i_2}) \cdot \ProbabilityMC<\MC, s_0>(s_{i_2}\dots s_n)
	\end{equation}
	The same holds analogously for any $\finitepath_2=s_0s_1\dots s_{i_2} \dots s_{i_2} \dots s_n\in\Finitepaths<\MC,g,2>$.

	We can then bound the probability that we wrongly estimated $\ProbabilityMC<\MC, s_0>$:


